SOAP: Style-Omniscient Animatable Portraits

Creating animatable 3D avatars from a single image remains challenging due to style limitations (realistic, cartoon, anime) and difficulties in handling accessories or hairstyles. While 3D diffusion models advance single-view reconstruction for general objects, outputs often lack animation controls or suffer from artifacts because of the domain gap. We propose SOAP, a style-omniscient framework to generate rigged, topology-consistent avatars from any portrait. Our method leverages a multiview diffusion model trained on 24K 3D heads with multiple styles and an adaptive optimization pipeline to deform the FLAME mesh while maintaining topology and rigging via differentiable rendering. The resulting textured avatars support FACS-based animation, integrate with eyeballs and teeth, and preserve details like braided hair or accessories. Extensive experiments demonstrate the superiority of our method over state-of-the-art techniques for both single-view head modeling and diffusion-based generation of Image-to-3D. Our code and data are publicly available for research purposes at https://github.com/TingtingLiao/soap.

==> figs/eye.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.35\textwidth]{figs/pdf/eye_reg.pdf}
    \caption{
        \textbf{Eyes}. The left two are the eyes in front and side view, while the right one shows the cross-section of the eyeball. The observed eye width is denoted as $l$. $\mathbf{c}$ and $\mathbf{r}$ are the eyeball center and radiance, respectively.  
    }
    \label{fig:eye-reg}
\end{figure}


==> figs/failure_cases.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.48\textwidth]{figs/pdf/failure_cases.pdf}
    \vspace{-0.5cm}
    \caption{  
        \textbf{Failure cases}. The reconstruction results with incorrect landmarks, erroneous \flame initialization, and inaccurate head parsing.    
    }
    \vspace{-0.5cm}
    \label{fig:failure}
\end{figure}


==> figs/tex_edit.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.48\textwidth]{figs/pdf/tex_edit.pdf}
    \vspace{-0.5cm}
    \caption{  
        Editable textures are enabled by the interpolated UV map. 
    }
    % \vspace{-0.5cm}
    \label{fig:tex_edit}
\end{figure}


==> sec/3_preliminary.tex <==
\section{Preliminary}
\label{sec:preliminary}
\flame \cite{FLAME:SiggraphAsia2017} is a parametric human head model. Given the shape $\beta$, pose $\theta$ and expression $\psi$ parameters, \flame models the human head as $\mathcal{F}(\beta, \theta, \psi)$:
\begin{align} 
\begin{split}
    \mathcal{F}(\beta, \theta, \psi) &= \mathbf{LBS}(\mathbf{M}(\beta, \theta, \psi), \mathrm{J}(\beta), \theta, \mathcal{W}) \\
    \mathbf{M}(\beta, \theta, \psi) &= \mathbf{T} + \mathrm{B_s}(\beta) + \mathrm{B_e}(\psi) + \mathrm{B_p}(\theta),  
\label{equ:flame}
\end{split}
\end{align}
where $\mathbf{T}$ is a t-pose, zero-shape template, $\mathrm{B_s}, \mathrm{B_e}$ and $\mathrm{B_p}$ are shape, expression and pose blendshapes, respectively. $\mathbf{M}$ is the template with blendshape offsets in canonical space. $\mathbf{LBS}$ is the linear blend skinning (LBS) function \cite{loper2023smpl}, that wraps $\mathbf{M}$ to the target pose with skinning weights $\mathcal{W}$ and joints $\mathrm{J}$. The joint locations are defined as 
\begin{align}
\mathrm{J}(\beta) &= \mathcal{J}(\mathbf{T} + \mathrm{B_s}(\beta)),
\label{equ:joint-mapping}
\end{align}
where $\mathcal{J}$ is a sparse matrix defining how to compute joint locations from mesh vertices. 

For simplify, we use $\kappa=(\beta,\theta,\psi)$ to denote shape, pose and expression, $\mathcal{B}=(\mathrm{B_s}, \mathrm{B_e}, \mathrm{B_p})$ denote the set of blending shape, and $\Omega=(\mathbf{T}, \mathbf{F}, \mathcal{W}, \mathcal{J}, \mathcal{B})$ to denote a rigged parametric model that can be control by $\kappa$, where $\mathbf{F}$ represents the triangles of $\mathbf{T}$. $\mathcal{F}(\Omega, {\kappa})$ denotes an avatar with specific shapes and poses. Previous methods \cite{Khakhulin2022ROME,yao2021deca,danvevcek2022emoca} typically apply varying values of $\kappa$ and introduce additional vertex offsets over $\mathcal{F}$ to model different shapes of 3D heads, while sharing the same rigging parameters $\Omega$. However, these methods tend to generate overly smooth results and struggle to model complex hairstyles and personal details due to the fixed topology and limited modeling ability of $\kappa$. To address these problems, \modelname, instead, learns personalized $\Omega$ for each identity.  

  

==> sec/4_method.tex <==
\section{Method}
\label{sec:method} 

\subsection{Overview}
Given a portrait image of a person, \modelname aims to build a well-rigged 3D avatars, with detailed geometry and all-around texture. However, the diversity in appearance and shape poses significant challenges for reconstructing a rigged avatar from style-agnostic portrait images. 

Our key insight addresses this challenge in two key aspects. To capture the texture or style diversity, we leverage the power of diffusion models to learn and generalize appearance in 2D space. To accommodate diverse shapes, we design an optimization process that adaptively deforms an initial shape to fit a wide range of geometries while preserving the semantic integrity of the head. For instance, the original mouth is deformed toward the target mouth instead of the nose. 

\modelname is summarized visually in Figure \ref{fig:pipeline}.  First, four orthogonal RGB images and normal images are generated from the input image using the multi-view diffusion models (Sec.~\ref{sec:multi-view-diffusion}). Next, we deform a \flame mesh $\mathcal{F}(\Omega,\kappa)$ to $\mathcal{F}(\Omega^*,\kappa)$ that aligns with the multi-view normals. (Sec.~\ref{sec:geometry}). Finally, we fit the eyeballs and teeth, and generate the UV texture using the multi-view RGB images (Sec.~\ref{sec:texturing}). 

 

% ==================================================
\subsection{Consistent Sparse-View Generation}
\label{sec:multi-view-diffusion}
Our multi-view image and normal diffusion model share the same network architecture as Unique3D \cite{wu2024unique3d}. We finetune them on the collected dataset including 19K 3D avatars (more details can be found in Sec.~\ref{sec:implement-details}). The multi-view image diffusion model takes a single image $\mathbf{I}\in \mathbb{R}^{256\times256\times3}$ as input and outputs four orthogonal RGB image $\mathcal{I}\in \mathbb{R}^{4\times256\times256\times3}$. The normal diffusion model then takes these four images $\mathcal{I}$ as input and generates the corresponding four normal images $\mathcal{N}\in \mathbb{R}^{4\times256\times256\times3}$.  To enhance visual quality, we employ a single-view super-resolution model to upscale the multi-view images and normals by a factor of four, achieving a resolution of 2048 without compromising multi-view consistency. 


% ==================================================
\subsection{Semantic Geometry and Rig Optimization}
\label{sec:geometry}
In this stage, our goal is to learn the geometry $\mathcal{F}(\Omega_{\mathbf{I}}, \mathcal{K}_{\mathbf{I}})$ that aligns with the target identity, where $\Omega_{\mathbf{I}}$ can be controlled by any given $\mathcal{K}$. To do so, we first optimize $\mathcal{K}_{\mathbf{I}}$ and the camera parameters $\pi$, which are fixed in subsequent steps. Then we adaptively deform $\mathcal{F}(\overline{\Omega}, \mathcal{K}_{\mathbf{I}})$ into $\mathcal{F}(\Omega_{\mathbf{I}}, \mathcal{K}_{\mathbf{I}})$ while preserving the semantic facial component of the head.  

As illustrated in Figure~\ref{fig:pipeline}, the personalized $\Omega_{\mathbf{I}}$ optimization involves the following steps: (1) semantic template deformation $\mathbf{T} \to$ \textcolor{blue}{$\mathbf{T}$}, where $\mathbf{T}$ and  \textcolor{blue}{$\mathbf{T}$} have the same number of vertices; (2) remeshing and rig interpolation $\Omega \to $ \textcolor{orange}{$\Omega$}; and (3) iteratively looping steps (1) and (2). 

\zheading{$\mathcal{K}_{\mathbf{I}}$ and Camera Optimization} Given an input image $\mathbf{I}$, a \flame mesh $\mathcal{F}(\Omega, \kappa)$ and camera $\pi$ are estimated by~\cite{danvevcek2022emoca}, and the facial landmarks $\mathbf{L} \in \mathbb{R}^{68\times 2}$ are detected by \cite{bulat2017far}. Utilizing the normal image $\mathcal{N}$ and landmarks $\mathbf{L}$, $\kappa$ and $\pi$ are further optimized. More details can be found in Appendix. 


\zheading{Semantic Template Deformation}   
Without constraints, the vertices may deform to arbitrary positions, disrupting the topology of the head, which is essential for animation. To preserve semantic consistency, we employ two key components: facial landmarks and head parsing masks, which help retain the semantic integrity of the head. The head parsing mask provides segmentation for three regions including the neck, face, and hair, while the facial landmarks offer detailed guidance for facial features, including the eyes, nose, lips, and jawline.

Specifically, the normal image is used to guide the template deformation, while $\mathbf{F}, \mathcal{W}, \mathcal{J}$, $\mathcal{B}$ and $\kappa$ remain fixed. During optimization, semantic constraints are applied to maintain the facial semantic topology, by encouraging the original facial parts (e.g., nose) to deform toward their corresponding target parts (e.g., nose). 
%We found that facial landmarks can effectively ensure the semantic topology for the face.

Given normal images $\mathcal{N}$, the initial mesh $\mathcal{F}(\Omega_0, \kappa)$, camera $\pi$, and landmarks $\mathbf{L}$, we iteratively update the template vertices $\mathbf{T}$ by aligning $\mathcal{F}(\Omega, \kappa)$ with $\mathcal{N}$. Specifically, we use the normal rendering loss $\mathcal{L}_{\mathrm{norm}}$, Laplacian regularization $\mathcal{L}_{\mathrm{lap}}$, landmark loss $\mathcal{L}_{\mathrm{lmk}}$ and eye loss $\mathcal{L}_{\mathrm{eye}}$:
\begin{align}
\begin{split}
\mathcal{L} &= \lambda_{\mathrm{norm}} \mathcal{L}_{\mathrm{norm}} +  \lambda_{\mathrm{lap}} \mathcal{L}_{\mathrm{lap}}  +  \lambda_{\mathrm{lmk}} \mathcal{L}_{\mathrm{lmk}} +  \lambda_{\mathrm{eye}} \mathcal{L}_{\mathrm{eye}} 
\end{split}
\end{align}
where $\lambda$ represents the weights to balance losses. 

\textit{Reconstruction Loss} We use the normal image as supervision to deform the template mesh and apply the Laplacian smoothing to regularize the surface meanwhile. The normal loss computes the difference between $\mathcal{N}$ and $\mathbf{n}$: 
\begin{align}
\mathcal{L}_{\mathrm{norm}}(\mathcal{N}, \mathbf{n}) = \sum \lambda_{\mathrm{MSE}}^{\mathbf{k}} \norm{\mathcal{N}_{\mathbf{k}}-\mathbf{n_k}}_{2}^{2}
\end{align}
where $\mathbf{n_k}$ is the rendered normal image of the 3D shape $\mathcal{F}(\Omega,\kappa)$ in view $\mathbf{k}\in \{ \mathrm{front}, \mathrm{left}, \mathrm{back}, \mathrm{right} \}$. $\lambda_{\mathrm{MSE}}$ is the weight of each view. 

\textit{Landmark Loss} We regularize the landmarks in both 2D and 3D spaces. Specifically, we utilize 2D facial landmarks detected from the image to guide the deformation process. Simultaneously, we enforce symmetry for the landmarks in the 3D space.
\begin{align}
\begin{split}
\mathcal{L}_{\mathrm{lmk}} = \mathcal{L}_{\mathrm{lmkpro}} + \mathcal{L}_{\mathrm{lmsym}}
\end{split}
\end{align}

The landmark loss computes the distance between the image landmarks $\mathbf{L}$ and the projected landmarks $\mathcal{P}(\hat{\mathbf{L}},\pi^{\mathrm{front}})\in \mathbb{R}^{68\times2}$. 
\begin{align}
\begin{split}
\mathcal{L}_{\mathrm{lmkpro}} &= ||\mathbf{L} - \mathcal{P}(\hat{\mathbf{L}},\pi^{\mathrm{front}})||_2^2  
\end{split}
\end{align}
where $\mathcal{P}$ is the projection operation, $\pi^{\mathrm{front}}$ denoting the input view camera, $\hat{\mathbf{L}} \in \mathbb{R}^{68\times 3}$ are the facial landmarks of $\mathcal{F}(\Omega,\kappa)$. Similar as Equation (\ref{equ:joint-mapping}), $\hat{\mathbf{L}}$ can be obtained by:   
\begin{align}
\begin{split}
&\hat{\mathbf{L}} = \mathbf{LBS} (\hat{\mathbf{L}}_{\mathrm{cano}}, J, \theta, \mathcal{W}) \\ 
&\hat{\mathbf{L}}_{\mathrm{cano}} = \mathcal{J}_{\mathrm{lmk}} (\mathbf{T}+\mathrm{B_s}(\beta)), 
\end{split}
\end{align}
where $\hat{\mathbf{L}}_{\mathrm{cano}}$ is the landmarks in canonical space (t-pose), mapped from $\mathbf{T}$ using the landmarks mapping matrix $\mathcal{J}_{\mathrm{lmk}} \in \mathbb{R} ^ {68\times |\mathbf{T}|}$ provided by \cite{FLAME:SiggraphAsia2017}. 

The symmetry landmark loss ensures the corresponding pairs of landmarks on opposite sides of the face are symmetric respect to the YZ-plane  for a frontal face. It is defined as:
\begin{align}
\begin{split} 
\mathcal{L}_{\mathrm{lmksym}} = \frac{1}{N} \sum_{i=1}^{N} \| \hat{\mathbf{L}}_{\mathrm{cano}}^{i} - \mathbf{R}(\hat{\mathbf{L}}_{\mathrm{cano}}^{j}) \|^2
\end{split}
\end{align}
Where $ \hat{\mathbf{L}}_{\mathrm{cano}}^{i}$ and $\hat{\mathbf{L}}_{\mathrm{cano}}^{j}$ represent a pair of symmetric landmark. $\mathbf{R}$  is the reflection transformation about the \( YZ \)-plane. 

% \input{figs/eye}

\qheading{Eyes Loss} We found that the eyeballs geometry tends to become concave if there is no constrain during optimization. This limits our ability to control the eye movements to some extent. To address this issue, we developed a strategy to ensure the eyeball geometry keeping convex. Specifically, we utilize the eye segmentation mask from the input image to ensure proper alignment of eyes area. Additionally, a regularization loss is applied to enforce the eyeball to be a spherical shape. 
\begin{align}
\mathcal{L}_{\mathrm{eye}} = \mathcal{L}_{\mathrm{eyesil}} + \mathcal{L}_{\mathrm{eyereg}} 
\end{align} 
Note we do not use the eye mask directly as supervision, since the rendered eyeball mask is always larger than the observed eye mask. Instead, we use the following loss: 
\begin{align}
\begin{split}
    \mathcal{L}_{\mathrm{eyesil}} =& \norm{\mathcal{S}_{\mathrm{e}} - \hat{\mathcal{S}}_\mathrm{e} \otimes \mathcal{S}_\mathrm{e} }_2^2 + \\
    & \norm{\hat{\mathcal{S}}_{\mathrm{ne}} - \mathcal{S}\otimes (1-\mathcal{S}_{\mathrm{e}})}_2^2
\end{split}
\end{align}
where $\otimes$ represents pixel-wise multiplication, $\mathcal{S}$ and $\mathcal{S}_{\mathrm{e}}$ denoting the ground truth image mask and eye mask respectively. $\hat{\mathcal{S}}_{\mathrm{e}}$ is the rendered eyeball mask for the eyeballs only, while $\hat{\mathcal{S}}_{\mathrm{ne}}$ is the rendered mask of the 3D shape $\mathcal{F}$ excluding the eyeballs. The first term ensures that the eyeballs are not smaller than the observed ones, while the second term enforces that vertices not belonging to the eyeballs lie outside the observed eyes area. 

Additionally, we approximate each eyeball as a sphere, defined by a center $\mathbf{c}$ and radius $\mathbf{r}$. The distance of every vertex on the sphere to the center should be equal to $\mathbf{r}$, formulated as: 
\begin{align}
\begin{split}
    &\mathcal{L}_{\mathrm{eyereg}}=\frac{1}{|\Theta|} \sum_{\mathbf{v} \in \Theta } \norm{\norm{\mathbf{v} - \mathbf{c}}_2^2 - \mathbf{r}}_2^2 \\ 
%      & \mathbf{c} = \mathbf{z} - \begin{bmatrix}
%  0\\
%  0\\
% \mathbf{r} \cos(\varepsilon / 2) 
% \end{bmatrix} , \, \mathbf{r}=\frac{l/2}{\sin(\varepsilon/2)} \\
    & \mathbf{c} = \mathbf{z} -  \left [ 0,0,\mathbf{r} \cos(\varepsilon / 2) \right ]^{\mathrm{T}}, \, \mathbf{r}=\frac{l/2}{\sin(\varepsilon/2)}
\end{split}
\end{align}
where $\Theta$ denotes the eyeball vertices. As illustrated in Figure \ref{fig:eye-reg}, $\varepsilon$ is the angle subtended by the eye, $\mathbf{z}$ is a reference point, $l$ is the average observed width of the left and right eyes in the input image. Note the left and right eyeballs share the same radius $\mathbf{r}$ but have different centers $\mathbf{c}$. For the reference point $\mathbf{z}$, we use the mean position of the selected eyelids vertices around each eyeball. 

\input{figs/diverse_avatars}

\zheading{Remeshing and Rig Interpolation}
After deformation, we remesh the template mesh from $\mathbf{T} \in \mathbb{R}^{\mathrm{N}\times3}, \mathbf{F} \in \mathbb{R}^{\mathrm{M}\times 3}$ to $\mathbf{T}' \in \mathbb{R}^{\mathrm{N'}\times3}, \mathbf{F}' \in \mathbb{R}^{\mathrm{M'}\times 3}$. 
%
The remeshing operation consists of three steps: subdividing large triangles with edges larger than $\epsilon$, flipping inconsistent triangles, and removing incorrect triangles. 
%
As the topology of the template mesh changes, the skinning weights $\mathcal{W}\in \mathbb{R}^{\mathrm{N}\times |\mathrm{J}|}$ and the joint mapping matrix $\mathcal{J} \in \mathbb{R}^{|\mathrm{J}|\times \mathrm{N}}$ also need to be updated accordingly. For skinning weights, we interpolate the value for the newly added vertex according to its neighbors:
%
\begin{align}
\mathcal{W}^k =  
\end{align}
%
We update the joint regressor matrix $\mathcal{J} \in \mathbb{R}^{}$ by 
%
\begin{align}
\mathcal{J} = \mathrm{J} (\mathbf{T} + \mathrm{B_s}({\beta}))^{-1},
\end{align}
%
where $\mathrm{J}$ is the canonical joints obtained from Equation \ref{equ:flame} using the newly deformed template. Our assumption is that the joints in canonical space does not change after remeshing.   

\subsection{Eyeballs, Teeth and Textures}
\label{sec:texturing}

